System Neural Diversity: Measuring Behavioral Heterogeneity in Multi-Agent Learning

Evolutionary science provides evidence that diversity confers resilience in natural systems. Yet, traditional multi-agent reinforcement learning techniques commonly enforce homogeneity to increase training sample efficiency. When a system of learning agents is not constrained to homogeneous policies, individuals may develop diverse behaviors, resulting in emergent complementarity that benefits the system. Despite this, there is a surprising lack of tools that quantify behavioral diversity. Such techniques would pave the way towards understanding the impact of diversity in collective artificial intelligence and enabling its control. In this paper, we introduce System Neural Diversity (SND): a measure of behavioral heterogeneity in multi-agent systems. We discuss and prove its theoretical properties, and compare it with alternate, state-of-the-art behavioral diversity metrics used in the robotics domain. Through simulations of a variety of cooperative multi-robot tasks, we show how our metric constitutes an important tool that enables measurement and control of behavioral heterogeneity. In dynamic tasks, where the problem is affected by repeated disturbances during training, we show that SND allows us to measure latent resilience skills acquired by the agents, while other proxies, such as task performance (reward), fail to. Finally, we show how the metric can be employed to control diversity, allowing us to enforce a desired heterogeneity set-point or range. We demonstrate how this paradigm can be used to bootstrap the exploration phase, finding optimal policies faster, thus enabling novel and more efficient MARL paradigms.

==> sections/discussion.tex <==

\begin{insight}
     \matteo{frame as heterogeneous is default}
     An $\mathrm{SND}$ of $0$ indicates that homogeneous training should be preferred to benefit from sample efficiency.
\end{insight}
\begin{insight}
\matteo{frame as confirmation snd is valid}
 An $\mathrm{SND}$ greater than $0$, when heterogeneous paradigms obtain higher rewards than homogeneous ones, indicates that heterogeneity enables performance.
\end{insight}
\begin{insight}
An $\mathrm{SND}$ greater than $0$, when homogeneous and heterogeneous paradigms obtain the same reward, indicates that heterogeneity enables resilience to noise.
\end{insight}
\begin{insight}
    In cases where the task undergoes repeated dynamic disruptions, SND is able to expose how heterogeneity allows agents to learn and maintain latent skills for resilience.
\end{insight}



%Behavioral diversity is a valuable skill in collective problems. Multi-agent systems that allow agents to specialize and learn unique (and potentially complementary) skills often demonstrate superior resilience towards disturbances~\cite{bettini2023hetgppo}.
This work has presented a novel framework for measuring behavioral heterogeneity with a System Neural Diversity (SND) metric. Our metric is able to measure behavioral diversity among agents with stochastic policies acting in a continuous state spaces.
We show, theoretically and empirically, that SND enables comparisons of diversity across different system sizes and provides a measure of behavioral redundancy.
These are two key properties that prior work (e.g., HSE) overlook, thus representing only a partial picture of system heterogeneity.
%Prior work in designing such diversity metrics has overlooked two key properties of interest -- the ability to compare diversity across varying team sizes, and the ability to represent redundancy. Our proposed metric unlocks these properties, and thus, proves to be a novel and complimentary tool that enables a direct measurement of heterogeneity.
%Our evaluations of the metric in a variety of multi-agent tasks (didactic and realistic) with different team sizes and different heterogeneity requirements establish the true representational power of our metric.
%We show in the \textit{Multi-Agent Goal Navigation} scenario that SND not only maintains an invariance to the number of agents in a team, but also captures a decrease in heterogeneity as more agents cluster into similar roles.
%This is in stark contrast with other state-of-the-art metrics (e.g., HSE) that do not demonstrate these properties, and taken independently, represent only a partial picture of system heterogeneity.
%\matteo{So this paragraph is saying the same as the one before. It seems a repetition to me. We could merge them and say: ``we have these 2 properties: a, b that others do not have. We prove them theoretically and showcase them empirically'', without mentioning the scenario name.}
Our evaluations of the metric in a variety of multi-robot tasks (didactic and realistic) with different system sizes and different heterogeneity requirements establish the true representational power of our metric.
The insights we draw from the various tasks indicate that SND provides a means to observe latent properties developed by a heterogeneous system during training, allowing a direct measurement of latent resilience, where other proxies, such as task performance (reward), fail to.
%In our static tasks, we show how our metric can act as a key diagnostic tool to analyze heterogeneous systems. In particular, we derive three insights from the comparison of SND with task reward. These insights suggest that SND can inform on the effectiveness of heterogeneous learning agents.
%In our dynamic tasks, where the problem is affected by a repeated disturbance during training, we show that heterogeneous agents are first able to learn specialized roles that allow them to cope with the disturbance, and then retain these roles even when the disturbance is removed.
%This is beneficial for the agents when the disturbance reoccurs.

Finally, while our evaluations suggest that heterogeneous training is a powerful paradigm for multi-agent problems, we caution that this may not always be the case.
%This is already evident in the \textit{Multi-Agent Goal Navigation} scenario when all agents are tasked towards the same goal.
%\autoref{fig:multi_goal_hom_v_het} shows that in this case, a homogeneous training offers an advantage in sample efficiency while achieving the same performance. Luckily, SND is able to measure the lack of heterogeneity in the task and can thus inform our choice (see Insight 1).
In fact, it is possible to construct pathological scenarios where, just like in nature~\cite{mckinney1997extinction}, excessive role specialization within a multi-agent system becomes the cause of failure during unforeseen changes.
For instance, highly specialized agents are not able to dynamically swap roles, and thus, without behavioral redundancy, the system performance may suffer from agent faults.
%in case no redundancy is present.
SND can still play an important role in such cases by aiding the analysis and regulation of a trade-off between specialization and redundancy.

%\aj{use a good example and maybe cite something similar in nature where role switching  kills a population..}


% We identify the following research questions --
% \aj{Need to workshop these questions to flow better. WIP.}
% \newline{}

% \textbf{RQ1.}
% \textit{Can a well-designed neural diversity metric inform the choice between heterogeneous vs homogeneous training?}
% \matteo{I would do: \textit{Can SND inform on the effectiveness of heterogeneous training?}}
% \newline{}
% We show that it does.
% In cases where the metric identifies a low diversity index for a heterogeneous training scenario, we deduce that the task structure did not have strong heterogeneity requirements.
% Thus, in these cases, a homogeneous training will produce the same results (good or bad) with a significantly higher sample efficiency.
% Conversely, in cases where the metric points to a larger diversity index for heterogeneous training, and yet the reward is comparable to the homogeneous counterpart, we posit that the diversity (task specialization, in this case) confers resilience to the team.

% \textbf{RQ2.}
% \textit{In cases where the task undergoes repeated dynamic disruptions .. }\newline{}
% \notes{.. can agents learn and retain diverse skills for resilience?}\newline{}
% \notes{.. can agents develop diverse/specialized skills and retained them for resilience?}
% \newline{}
% Yes, we show that heterogeneity contributes to latent resilience that a team can later employ when the disruptions recur.


% \textbf{RQ3(?).}
% \textit{Given the choice, should heterogeneity be always preferred?}
% \matteo{I like this. Dunno if we can answer it in this paper tho :(}
% \newline{}
% We think not.
% We identfy counter-examples where switching the roles (`identities') of the agents proves behavior specialization to be in fact detrimental.
% We also show that the nature of the task and the degree of heterogeneity determines, in part, the amount of degradation observed.


